Synchronization in Complex Oscillator Networks and Smart Grids

The emergence of synchronization in a network of coupled oscillators is a fascinating topic in various scientific disciplines. A coupled oscillator network is characterized by a population of heterogeneous oscillators and a graph describing the interaction among them. It is known that a strongly coupled and sufficiently homogeneous network synchronizes, but the exact threshold from incoherence to synchrony is unknown. Here we present a novel, concise, and closed-form condition for synchronization of the fully nonlinear, non-equilibrium, and dynamic network. Our synchronization condition can be stated elegantly in terms of the network topology and parameters, or equivalently in terms of an intuitive, linear, and static auxiliary system. Our results significantly improve upon the existing conditions advocated thus far, they are provably exact for various interesting network topologies and parameters, they are statistically correct for almost all networks, and they can be applied equally to synchronization phenomena arising in physics and biology as well as in engineered oscillator networks such as electric power networks. We illustrate the validity, the accuracy, and the practical applicability of our results in complex networks scenarios and in smart grid applications.

==> Manuscript/statistics.tex <==
The synchronization conditions \eqref{eq: sync condition - sufficient} and \eqref{eq: sync condition - necessary} are simple scalar quantities for arbitrary connected network topologies and for all possible parameter values. This fact is both miraculous and surprising, and it poses a major challenge on how to explore the vast parameter space. 

Generally, we observe that the sufficient bound \eqref{eq: sync condition - sufficient} seems to be accurate for a sparse topology and the necessary bound \eqref{eq: sync condition - necessary} becomes more accurate as the graph becomes denser and number of oscillators increases. 
%
In order to illustrate and test this hypothesis in a low-dimensional parameter space, we simulate the first-order model \eqref{eq: topological Kuramoto model} with  coupling gain $K>0$, uniform coupling weights $a_{ij}=1$, and a one-parameter family of Erd\"os-R\'enyi random graph models. Given our insight form the standard Kuramoto model \citepri{SI-FD-FB:10w}, the two extreme distributions are the bipolar distribution and the uniform distribution corresponding to the largest and smallest coupling. 
%
Figure \ref{Fig: Simulation -- ER random graph - topology} illustrates our findings for an Erd\"os-R\'enyi random graph model with probability $p \in {[0.15,1]}$ of connecting two nodes, and for the two cases of a bipolar distribution and a uniform distribution supported for $\omega_{i}\in{[-1,1]}$. In Figure \ref{Fig: Simulation -- ER random graph - topology}, the value of $K$ is the exact critical coupling (found numerically) for which stable synchronization manifolds exist, and each data point in Figure \ref{Fig: Simulation -- ER random graph - topology} corresponds to the mean value over 100 simulations, with randomized initial conditions, a random graph realization with parameter $p$, and natural frequencies $\omega_{i}$ sampled from a distribution supported the compact interval ${[-1,1]}$. 

\begin{figure}
  \centering
  \includegraphics[scale=0.44]{./Pictures/ER}
    \caption{Critical coupling strength for $n$ coupled oscillators obeying the dynamics \eqref{eq: topological Kuramoto model} and coupled in a random Erd\"os-R\'enyi network with parameter $p$. The values of $\omega_{i}$ are sampled from either a bipolar distribution {\bf (a)} or a uniform distribution {\bf (b)} supported for $\omega_{i} \in {[-1,1]}$.}
     \label{Fig: Simulation -- ER random graph - topology}
\end{figure}

Figure \ref{Fig: Simulation -- ER random graph - topology} shows that the sufficient condition \eqref{eq: sync condition - sufficient} is extremely accurate for a sparsely connected graph, that is, for small $p$ and $n$. This accuracy for sparse graphs is not surprising since the condition \eqref{eq: sync condition - sufficient} is exact for a tree, the sparsest possible connected graph.
%can typically be reduced to multiple clusters which are one-connected among each other
%The effective resistance between these one-connected clusters is equivalent to the weight $1/K$ of the single edge interconnecting these clusters which has to dominate the non-uniformity according to condition \eqref{eq: equivalent resistive condition}.
%
Likewise, the results are not surprising for a sufficiently dense graph, that is, for large $p \approx 1$. In this case, the graph is nearly complete, and the obtained results confirm the results known for classical Kuramoto case \citepri{SI-FD-FB:10w}: for a bipolar distribution the sufficient condition \eqref{eq: sync condition - sufficient} is exact (see (a)), and, analogously, the complete graph case predicts a small critical coupling for a uniform distribution (see (b)). Surprisingly, for the bipolar distribution the smallest coupling gain is required for the intermediate regime of neither sparse nor dense graphs.
% discuss 4/pi(!!!!)
%
Furthermore, the necessary condition \eqref{eq: sync condition - necessary} becomes more accurate for increasing number $n$ of oscillators and for sufficiently sparse (a) or dense (b) graphs.

In order to test the sensitivity of the synchronization condition \eqref{eq: sync condition - sufficient} with respect to a non-uniformity in the weighting of a graph, we simulate the the first-order model \eqref{eq: topological Kuramoto model} for the prototypical example of an Erd\"os-R\'enyi random graph with $n=30$ nodes, random graph parameter $p = 0.4$, and for randomized weightings $a_{ij}$ of the coupling weights sampled from a uniform distribution supported on ${[1 - \epsilon , 1 + \epsilon]}$. 
%The natural frequencies are sampled from distributions of varying width $\Lambda$. 
%
Rather than using the coupling gain $K$ as a control parameter to uniformly change all coupling weights as $K \cdot a_{ij}$ in order to find the synchronization treshold, we used a unit coupling gain $K=1$, discarded simulations that did not reach synchronization, and only counted converging simulations. Our findings are reported in Figure \ref{Fig: Simulation -- ER random graph - weighting}, where each data point corresponds to the mean value and the standard deviation of $\|B^{T} L^{\dagger} \omega\|_{\infty}$ over 100 convergent simulations.
%
\begin{figure}
  \centering
  \includegraphics[scale=0.44]{./Pictures/ER-Weights}
    \caption{Mean values and standard deviation of $\|B^{T} L^{\dagger} \omega\|_{\infty}$ for $n=30$ coupled oscillators obeying the dynamics \eqref{eq: topological Kuramoto model} and coupled in a random Erd\"os-R\'enyi network with parameter $p=0.4$. The values of $\omega_{i}$ are sampled from either a bipolar distribution (a) or a uniform distribution (b) with width $\Lambda$, and the weights $a_{ij}$ are sampled from a uniform distribution supported on ${[1 - \epsilon , 1 + \epsilon]}$.}
     \label{Fig: Simulation -- ER random graph - weighting}
\end{figure}
%
Surprisingly, both the mean value and the standard deviation of $\|B^{T} L^{\dagger} \omega\|_{\infty}$ appear to be independent of the parameter $\epsilon$ specifying the width of the weighting distribution. As expected, the mean value and the standard deviation increase with the width $\Lambda$ of the distribution of natural frequencies $\omega_{i}$, that is, they rather depend on the ``stress'' over the edges in the network. 

We draw the following conclusions from the statistical studies presented in this section: 
%
First, for a sparse topology the sufficient condition \eqref{eq: sync condition - sufficient} is extremely close to the exact synchronization threshold. 
%
Second, as the graph becomes denser and number of oscillators increases the necessary condition \eqref{eq: sync condition - necessary} becomes more accurate for a uniform distribution of the natural frequencies and less accurate for a bipolar distribution of the natural frequencies. Third, the  synchronization conditions appear to be independent of non-uniform weightings in the graph.
%
Finally, we remark the conclusions drawn from Figure \ref{Fig: Simulation -- ER random graph - topology} and Figure \ref{Fig: Simulation -- ER random graph - weighting} can also be drawn for other one-parameter families of random graphs, such as random geometric graphs investigated in the supplementary information.
